An Integrated Approach for Failure Mitigation & Localization in Power Systems

The transmission grid is often comprised of several control areas that are connected by multiple tie lines in a mesh structure for reliability. It is also well-known that line failures can propagate non-locally and redundancy can exacerbate cascading. In this paper, we propose an integrated approach to grid reliability that (i) judiciously switches off a small number of tie lines so that the control areas are connected in a tree structure; and (ii) leverages a unified frequency control paradigm to provide congestion management in real time. Even though the proposed topology reduces redundancy, the integration of tree structure at regional level and real-time congestion management can provide stronger guarantees on failure localization and mitigation. We illustrate our approach on the IEEE 39-bus network and evaluate its performance on the IEEE 118-bus, 179-bus, 200-bus and 240-bus networks with various network congestion conditions. Simulations show that, compared with the traditional approach, our approach not only prevents load shedding in more failure scenarios, but also incurs smaller amounts of load loss in scenarios where load shedding is inevitable. Moreover, generators under our approach adjust their operations more actively and efficiently in a local manner.

==> case_study_v1.tex <==
We now use present case studies using the IEEE 39, 118, 179, 200, and 240 bus networks to illustrate the performance of our integrated approach. 

\subsection{Dynamic Demonstration}
\begin{figure}[t]
\centering
\includegraphics[width=.4\textwidth]{fig/grid_39.png}
\caption{IEEE 39-bus network with two control areas from \cite{zhao2016unified}. Blue tie lines are switched off to create a tree structure with bridge $(2,3)$.}\label{fig:grid_39}
\end{figure}
We first illustrate the dynamic process of our proposed approach for the IEEE 39-bus network whose parameters are adapted from \cite{zhao2016unified}. It consists of two control regions, which are connected by three tie lines, namely $(1,2)$, $(2,3)$ and $(26,27)$.

We switch off the tie lines $(1,2)$ and $(26,27)$, chosen heuristically as those with the smallest absolute flow. Two control regions are then connected in a tree structure as shown in Fig.~\ref{fig:grid_39}. 
We implement the unified control on all nodes as follows. We only allow to adjust generations at first, but, if a severe failure is detected, the controller is then allowed to reduce loads. As a last resort, zero area control error can be lifted. The threshold is set to $0.5$pu for dual variables.

As illustrated in Fig.~\ref{fig:non_severe}, in the case of the non-severe failure $(4,14)$, the dual variables are always below the threshold and the system quickly converges to a safe equilibrium. On the other hand, the failure $(6,7)$ leads to unstable oscillations of dual variables and a severe warning is raised at $10$ sec, as depicted in Fig.~\ref{fig:severe}. The controller is then allowed to shed loads, action that quickly restabilizes the system. Note that the flow on line $(25,26)$ remains unchanged at steady state for both failures, as it belongs to a non-associated region.

\begin{figure}[!h]
%\vspace{-0.8cm}
\centering
\subfloat[Dual variable dynamics\label{fig:non_severe_dual}] {\includegraphics[width=.24\textwidth]{fig/non_severe_dual_eps}}
\hfill
\subfloat[Line flow dynamics\label{fig:non_severe_flow}] {\includegraphics[width=.24\textwidth]{fig/non_severe_flow_eps}}
\caption{System dynamics after the non-severe failure of line $(4,14)$. The controller is only allowed to reduce generations.}
\label{fig:non_severe}
\end{figure}
\begin{figure}[!h]
%\vspace{-0.8cm}
\centering
\subfloat[Dual variable dynamics\label{fig:severe_dual}] {\includegraphics[width=.24\textwidth]{fig/severe_dual_eps}}
\hfill
\subfloat[Line flow dynamics\label{fig:severe_flow}] {\includegraphics[width=.24\textwidth]{fig/severe_flow_eps}}
\caption{System dynamics after the severe failure of line $(6,7)$. A warning is raised at time $10$ sec, at which point the controller is allowed to shed loads.}
\label{fig:severe}
\end{figure}

% \begin{table*}
% \def\arraystretch{1.3}
% \centering
% \caption{Number of scenarios with non-zero LLR/AGR over test networks.} \label{table:stat1}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% & &\multicolumn{3}{c|}{UC + mesh}&\multicolumn{3}{c|}{UC + tree} & \multicolumn{3}{c|}{AGC + mesh} & \multicolumn{3}{c|}{AGC + tree}\\
% \hline
% case & $\alpha$ & 0.1 & 1 & 10 & 0.1 & 1 & 10 & 0.1 & 1 & 10 & 0.1 & 1 & 10 \\
% \hline
% \multirow{2}{*}{118}& LLR &  96.15\% & 6.04\% & 2.20\% & 93.41\% & 8.24\% & 2.75\% & 98.90\% & 26.37\% & 2.20\% & 96.69\% & 50.00\% & 2.75\%\\
% \cline{2-14}
% &AGR & 98.90\% & 31.87\% & 3.85\% & 96.70\% & 55.49\% & 4.40\% & 98.90\% & 26.92\% & 3.85\% & 96.69\% & 54.40\% & 4.40\%\\
% \hline
% \multirow{2}{*}{179}& LLR & 35.14\% & 2.70\% & 0.77\% & 38.61\% & 2.70\% & 0.77\% & 91.47\% & 4.63\% & 0.77\% & 93.41\% & 6.18\% & 0.77\%\\
% \cline{2-14}
% &AGR & 90.73\% & 79.54\% & 16.22\% & 93.44\% & 44.02\% & 19.31\% & 91.47\% & 63.32\% & 16.22\% & 93.41\% & 38.22\% & 19.31\%\\
% \hline
% \multirow{2}{*}{200}& LLR & 90.56\% & 10.30\% & 9.87\% & 90.99\% & 21.03\% & 17.17\% & 93.99\% & 10.30\% & 9.87\% & 92.58\% & 39.66\% & 17.17\%\\
% \cline{2-14}
% &AGR & 93.99\% & 23.61\% & 23.61\% & 92.70\% & 50.64\% & 34.33\% & 93.99\% & 23.61\% & 23.61\% & 92.58\% & 50.43\% & 34.33\%\\
% \hline
% \multirow{2}{*}{240}& LLR & 92.22\% & 7.53\% & 0.23\% & 83.07\% & 8.94\% & 0.46\% & 98.59\% & 94.74\% & 0.23\% & 98.08\% & 73.00\% & 0.46\%\\
% \cline{2-14}
% &AGR & 98.63\% & 94.98\% & 11.87\% & 98.63\% & 86.01\% & 13.01\% & 98.59\% & 94.97\% & 11.87\% & 98.56\% & 86.50\% & 13.01\%\\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}
% \def\arraystretch{1.3}
% \centering
% \caption{Average values of non-zero LLR/AGR over test networks.} \label{table:stat1}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% & &\multicolumn{3}{c|}{UC + mesh}&\multicolumn{3}{c|}{UC + tree} & \multicolumn{3}{c|}{AGC + mesh} & \multicolumn{3}{c|}{AGC + tree}\\
% \hline
% case & $\alpha$ & 0.1 & 1 & 10 & 0.1 & 1 & 10 & 0.1 & 1 & 10 & 0.1 & 1 & 10 \\
% \hline
% \multirow{4}{*}{118}& LLR (!=0) & 2.42\% & 2.65\% & 1.55\% & 2.05\% & 2.34\% & 1.36\% & 29.98\% & 4.64\% & 1.55\% & 24.50\% & 4.22\% & 1.36\%\\
% \cline{2-14}
% & LLR (all) & 2.33\% & 0.16\% & 0.03\% & 1.91\% & 0.19\% & 0.04\% & 29.65\% & 1.22\% & 0.03\% & 23.69\% & 2.11\% & 0.04\% \\
% \cline{2-14}
% &AGR (!=0) & 20.97\% & 17.75\% & 21.43\% & 14.57\% & 14.92\% & 20.83\% & 24.33\% & 22.03\% & 21.43\% & 27.23\% & 28.25\% & 21.30\%\\
% \cline{2-14}
% & AGR (all) & 20.74\% & 5.66\% & 0.82\% & 14.09\% & 8.28\% & 0.92\% & 24.06\% & 5.93\% & 0.82\% & 26.32\% & 15.36\% & 0.94\% \\
% \hline
% \multirow{3}{*}{179}& LLR & 1.43\% & 1.44\% & 0.13\% & 1.34\% & 1.44\% & 0.13\% & 14.12\% & 2.90\% & 0.13\% & 14.48\% & 1.96\% & 0.13\%\\
% \cline{2-14}
% &AGR (!=0)& 56.05\% & 58.82\% & 70.28\% & 70.60\% & 75.32\% & 70.55\% & 77.26\% & 89.87\% & 75.12\% & 79.15\% & 86.31\% & 68.76\%\\
% \cline{2-14}
% & AGR (all) & 50.86\% & 46.78\% & 11.40\% & 65.97\% & 33.15\% & 13.62\% & 70.68\% & 56.90\% & 12.18\% & 73.94\% & 32.99\% & 13.27\% \\
% \hline
% \multirow{3}{*}{200}& LLR & 4.19\% & 1.41\% & 0.75\% & 3.57\% & 1.83\% & 1.06\% & 40.33\% & 1.41\% & 0.75\% & 40.48\% & 9.30\% & 1.06\%\\
% \cline{2-14}
% &AGR (!=0) & 51.99\% & 40.19\% & 51.10\% & 32.76\% & 43.82\% & 50.72\% & 76.06\% & 42.49\% & 50.81\% & 53.34\% & 55.40\% & 50.82\%\\
% \cline{2-14}
% &AGR (all) & 48.87\% & 9.49\% & 12.06\% & 30.37\% & 22.19\% & 17.42\% & 71.49\% & 10.03\% & 11.99\% & 49.38\% & 27.94\% & 17.45\% \\
% \hline
% \multirow{3}{*}{240}& LLR & 0.83\% & 1.64\% & 1.01\% & 0.77\% & 1.32\% & 0.61\% & 15.89\% & 5.54\% & 1.01\% & 10.11\% & 7.17\% & 0.61\%\\
% \cline{2-14}
% &AGR (!=0) & 52.51\% & 51.39\% & 93.76\% & 59.18\% & 43.89\% & 89.90\% & 65.60\% & 57.33\% & 96.15\% & 83.30\% & 56.81\% & 93.05\%\\
% \cline{2-14}
% & AGR (all) & 51.79\% & 48.81\% & 11.13\% & 58.37\% & 37.75\% & 11.70\% & 64.67\% & 54.44\% & 11.42\% & 82.10\% & 49.14\% & 12.11\% \\
% \hline
% \end{tabular}
% \end{table*}




\subsection{Statistics on Failure Mitigation}
%\cliang{Table 1 is too condensed. Probably easier to separate into two tables.}
%\lguo{I agree Table 1 is a bit dense, for two reasons: (1) Each cell contains a pair of values, which the reader will have to read through corresponding text to know which value is from which; (2) The values for number of scenarios are plain cardinality number, yet the values for average LLR/AGR should be interpreted as a percentile - this may be confusing at first glance. I have separated the table into two tables covering number of scenarios and average value respectively (original table still in commented section), and reordered the table labels, which hopefully address these two issues.}
%\cliang{Thanks Daniel. It looks much more clear now.}


% \cliang{Reviewers suggest to evaluate the UC and tree partitioning individually -- especially to show that tree partition is necessary.}

% \cliang{Lossless assumption \& DC assumption. Should we include some AC results as well?}

% \cliang{More simulation results from Shuyue.}

% \lguo{Are these simulations already finished? If so, we can consider adding them here (provided that they will not be repeated in SmartGridComm paper). If not, then let us not worry too much about adding new sections here given the amount of time we have.}
% \cliang{Still waiting for the updated results...}

% \cliang{TBA: results on case 118, 176, 200, 240 networks with AGC + original network, AGC + revised network, UC + original network, UC + revised network...}

% \cliang{TBD: simulations to validate that tree partitioning will not limit the grid transfer capacity. }

We now evaluate the mitigation performance of our proposed approach on the IEEE 118-bus, 179-bus, 200-bus and 240-bus networks. For each network, we first partition it into two control regions using network modularity clustering algorithm as proposed in \cite{zocca2019or}. We then keep the tie line with the largest absolute flow as the remaining bridge connecting these two regions, and switch off other tie lines between these two regions. 
Basic statistics on the original networks are summarized in Table~\ref{table:stat_network}.
\begin{table}[!t]
\def\arraystretch{1.3}
\centering
\caption{Statistics on original networks.} \label{table:stat_network}
\begin{tabular}{|c|c|c|c|}
\hline
Network & \# of Edges & Region Size & \# of Tie Lines  \\
\hline
118 & 186 & (83, 35) & 4 \\
\hline
179 & 263 & (98, 81) & 4\\
\hline
200 & 242 & (103, 94) & 9 \\
\hline
240 & 448 & (143, 97) & 10\\
\hline
\end{tabular}
\end{table}

Our proposed approach consists of two key components: a tree structure at regional level and a unified controller for real-time response. In order to showcase their contributions separately, we compare the system performance against failures with the following four mitigation strategies:
{
\renewcommand{\theenumi}{S\arabic{enumi}}
\begin{enumerate}
    \item Unified controller (UC) on tree-connected regions;
    \item Unified controller (UC) on mesh-connected regions;
    \item Automatic generation control (AGC)\footnote{We model AGC as an algorithm that solves \eqref{eqn:uc_olc} without enforcing line flow limits \eqref{eqn:line_limit}.} on tree-connected regions;
    \item Automatic generation control (AGC) on mesh-connected regions;
\end{enumerate}
}

The simulated scenarios are created as follows. For each network, we first adopt the nominal demand profile from \cite{babaeinejadsarookolaee2019power} and obtain an initial operating point through a certain DC OPF on the original network. 
The power injections from this DC OPF problem are used for all mitigation strategies S1, S2, S3, S4. The resulting line flows will generally be different depending on whether the network is tree partitioined or not.
Next, we iterate over every transmission line as initial failures and simulate the cascading processes under the aforementioned four strategies. Moreover, to test their performance under various network congestion conditions, we scale the line flow limit and generation limit by a common factor $\alpha=0.5, 1, 1.5$. For a fair comparison, all four strategies follow the same relaxation procedure as described in the previous subsection when the optimization is infeasible. We remark that since AGC does not enforce line  limits, the cascading failure may proceed for multiple stages as described in Section~\ref{section:pre}, while UC is guaranteed to terminate the failure at the first stage.



We quantify the mitigation performance using the \textit{load loss rate} (LLR), defined as the ratio of the total loss of load to the total demand. The localization performance is evaluated by the \textit{adjusted generator rate} (AGR) which is the ratio of the number of generators whose operating points have changed after the failures to the total number of generators. The range for both LLR and AGR is between $[0,100\%]$, and a smaller value indicates better mitigation/localization performance.
%\slow{Should the AGR ratio in Table I be between $[0, 100\%]$?  }
Tables~\ref{table:stat1} and \ref{table:stat2} summarize our results for all test networks with different congestion conditions. For each of them, we compare these two metrics under aforementioned strategies.
More specifically, we show two values for each metric: (i) the percentile ratio between the number of scenarios with non-zero LLR/AGR and the total scenarios in Table~\ref{table:stat1}, and (ii) the average value among those scenarios in Table~\ref{table:stat2}.
% More specifically, we show two numbers for each metric $\calM$: (i) the number of failure scenarios with non-zero $\calM$; and (ii) the average $\calM$ among scenarios with non-zero $\calM$.

\subsubsection{Effect of Unified Controller}
Compared with AGC based strategies (S3 and S4), when UC is adopted at real time (S1 and S2), both the frequency and severity of load loss is strictly lower for all test network over all congestion conditions. Moreover, generator adjust their operations more actively and efficiently under UC based strategies. Specifically, when the congestion is less severe (larger $\alpha$), S1 and S2 tend to adjust their generators in more scenarios and lead to significantly less load loss. 
When the congestion becomes worse, however, S3 and S4 lead to slightly more scenarios with non-zero AGR but much higher LLR. This is because generators under AGC based strategies are only passively affected to stabilize the grid as the cascading process keeps unfolding.

\subsubsection{Effect of Tree Structure}
Compared with strategies over mesh-connected regions (S2 and S4), tree structure based strategies (S1 and S3), which aim to improve grid reliability through better failure localization, indeed achieve slightly lower LLR for most congestion conditions on 118-bus, 179-bus and 240-bus networks. Mesh structure based strategies on 200-bus network, however, yields less load loss. A possible explanation might be that 200-bus network is already very sparse and tie line switching further downgrades the grid reliability. More importantly, when UC operates over a tree structure (S1), fewer generations are affected compared to the mesh structure (S2), indicating a better localization performance against failures.

In summary, our approach (S1) not only prevents most failures from causing any loss of load, but also significantly reduces the amount of load loss when load shedding is inevitable. This improvement is particularly remarkable when the grid becomes congested. In terms of localization performance, generators adjust their operations more actively and efficiently, and only generators within associated regions are affected for most failure scenarios.

%\begin{table}[!t]
%\def\arraystretch{1.3}
%\centering
%\caption{Statistics on load loss rate and number of adjusted generators. First number in each cell is from the proposed approach, while the second number is from AGC.} \label{table:stat}
%\begin{tabular}{|p{0.45cm}|c|c|c|c|c|}
%\hline
% &$(\alpha,\beta)$ &$(0.8, 0.8)$ & $(0.7, 0.8)$ & $(0.65, 0.8)$ &$(0.65, 0.5)$  \\
%\hline
%\multirow{2}{*}{LLR} & Scen. & 97, 124 & 101, 499 & 123, 2398 & 144, 2476\\
%\cline{2-6}
%& Avg. & 1.08, 2.23 & 1.04, 6.50 & 0.87, 6.44 & 0.98, 7.92 \\
%\hline
%\multirow{2}{*}{AGR} & Scen. & 553, 390 & 790, 794 & 1301, 2695 & 1308, 2744\\
%\cline{2-6}
%& Avg. & 31.5, 45.2 & 28.1, 58.0 & 23.1, 77.6 & 21.9, 70.0 \\
%\hline
%\end{tabular}
%\end{table}
% \begin{table*}
% \def\arraystretch{1.3}
% \centering
% \caption{Fraction of failure scenarios with non-zero LLR/AGR over test networks. Threshold: 0.01\%} \label{table:stat1}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% & &\multicolumn{3}{c|}{UC + Tree}&\multicolumn{3}{c|}{UC + Mesh} & \multicolumn{3}{c|}{AGC + Tree} & \multicolumn{3}{c|}{AGC + Mesh}\\
% \hline
% Network & $\alpha$ & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 \\
% \hline
% \multirow{2}{*}{118}& LLR &  63.69\% & 8.24\% & 4.95\% & 45.25\% & 6.04\% & 2.75\% & 96.65\% & 50.00\% & 4.95\% & 98.88\% & 26.37\% & 3.85\%\\
% \cline{2-14}
% &AGR & 94.41\% & 52.75\% & 8.24\% & 96.09\% & 31.87\% & 6.59\% & 96.65\% & 54.40\% & 8.24\% & 98.88\% & 26.92\% & 6.59\%\\
% \hline
% \multirow{2}{*}{179}& LLR & 4.26\% & 2.70\% & 1.93\% & 4.26\% & 2.70\% & 1.93\% & 71.32\% & 6.18\% & 3.09\% & 80.62\% & 4.63\% & 2.54\%\\
% \cline{2-14}
% &AGR & 71.32\% & 44.02\% & 37.07\% & 74.42\% & 69.88\% & 21.24\% & 78.29\% & 38.22\% & 24.71\% & 83.72\% & 63.32\% & 19.69\%\\
% \hline
% \multirow{2}{*}{200}& LLR & 23.28\% & 21.12\% & 17.60\% & 12.07\% & 10.34\% & 9.87\% & 53.45\% & 39.66\% & 17.60\% & 26.72\% & 10.34\% & 9.87\%\\
% \cline{2-14}
% &AGR & 56.03\% & 47.41\% & 31.33\% & 36.21\% & 20.26\% & 20.60\% & 56.90\% & 47.41\% & 31.33\% & 36.64\% & 20.26\% & 20.60\%\\
% \hline
% \multirow{2}{*}{240}& LLR & 26.46\% & 8.99\% & 2.51\% & 25.76\% & 7.60\% & 2.28\% & 97.19\% & 72.81\% & 3.20\% & 98.13\% & 94.70\% & 2.74\%\\
% \cline{2-14}
% &AGR & 94.61\% & 73.73\% & 21.92\% & 96.72\% & 91.47\% & 16.67\% & 97.66\% & 86.41\% & 18.72\% & 98.13\% & 94.93\% & 15.53\%\\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}
% \def\arraystretch{1.3}
% \centering
% \caption{Average values of non-zero LLR/AGR over test networks. Threshold: 0.01\%} \label{table:stat2}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% & &\multicolumn{3}{c|}{UC + Tree}&\multicolumn{3}{c|}{UC + Mesh} & \multicolumn{3}{c|}{AGC + Tree} & \multicolumn{3}{c|}{AGC + Mesh}\\
% \hline
% Network & $\alpha$ & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 \\
% \hline
% \multirow{2}{*}{118}& LLR & 1.22\% & 2.34\% & 1.05\% & 2.15\% & 2.65\% & 1.29\% & 17.69\% & 4.22\% & 3.28\% & 18.80\% & 4.64\% & 3.82\%\\
% \cline{2-14}
% &AGR& 10.37\% & 12.15\% & 15.68\% & 17.68\% & 15.20\% & 18.06\% & 14.56\% & 15.15\% & 16.54\% & 20.52\% & 15.38\% & 17.59\%\\
% \hline
% \multirow{2}{*}{179}& LLR & 1.44\% & 1.44\% & 1.37\% & 1.42\% & 1.44\% & 1.37\% & 3.18\% & 1.96\% & 1.83\% & 3.94\% & 2.90\% & 1.78\%\\
% \cline{2-14}
% &AGR & 26.52\% & 26.80\% & 36.71\% & 41.45\% & 42.35\% & 46.39\% & 58.30\% & 62.07\% & 38.79\% & 73.96\% & 75.15\% & 38.67\%\\
% \hline
% \multirow{2}{*}{200}& LLR  & 2.59\% & 1.83\% & 1.13\% & 2.32\% & 1.41\% & 0.75\% & 16.51\% & 9.30\% & 1.13\% & 12.38\% & 1.41\% & 0.75\%\\
% \cline{2-14}
% &AGR & 29.86\% & 36.05\% & 50.61\% & 39.94\% & 35.89\% & 50.66\% & 50.42\% & 45.43\% & 50.61\% & 49.57\% & 35.89\% & 50.66\%\\
% \hline
% \multirow{2}{*}{240}& LLR& 0.79\% & 1.32\% & 2.09\% & 0.94\% & 1.64\% & 2.24\% & 9.34\% & 7.19\% & 2.77\% & 9.76\% & 5.53\% & 3.06\%\\
% \cline{2-14}
% &AGR & 24.47\% & 21.52\% & 51.93\% & 40.62\% & 45.50\% & 66.24\% & 49.49\% & 50.42\% & 51.61\% & 60.43\% & 56.17\% & 63.12\% \\
% \hline
% \end{tabular}
% \end{table*}


\begin{table*}
\def\arraystretch{1.3}
\centering
\caption{Fraction of failure scenarios with non-zero LLR/AGR over test networks.} \label{table:stat1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
& &\multicolumn{3}{c|}{UC + Tree}&\multicolumn{3}{c|}{UC + Mesh} & \multicolumn{3}{c|}{AGC + Tree} & \multicolumn{3}{c|}{AGC + Mesh}\\
\hline
Network & $\alpha$ & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 \\
\hline
\multirow{2}{*}{118}& LLR &  48.60\% & 8.24\% & 4.95\% & 43.02\% & 6.04\% & 2.75\% & 96.65\% & 50.00\% & 4.95\% & 98.88\% & 26.37\% & 3.85\%\\
\cline{2-14}
&AGR & 94.41\% & 52.75\% & 8.24\% & 96.09\% & 31.87\% & 6.59\% & 96.65\% & 54.40\% & 8.24\% & 98.88\% & 26.92\% & 6.59\%\\
\hline
\multirow{2}{*}{179}& LLR & 3.88\% & 2.32\% & 1.54\% & 3.88\% & 2.32\% & 1.54\% & 68.22\% & 3.86\% & 2.32\% & 58.53\% & 4.25\% & 2.16\%\\
\cline{2-14}
&AGR & 71.32\% & 44.02\% & 37.07\% & 74.42\% & 69.88\% & 21.24\% & 78.29\% & 38.22\% & 24.71\% & 83.72\% & 63.32\% & 19.69\%\\
\hline
\multirow{2}{*}{200}& LLR & 21.12\% & 18.53\% & 15.02\% & 9.48\% & 7.76\% & 7.30\% & 51.29\% & 37.07\% & 15.02\% & 24.14\% & 7.76\% & 7.30\%\\
\cline{2-14}
&AGR & 56.03\% & 47.41\% & 31.33\% & 36.21\% & 20.26\% & 20.60\% & 56.90\% & 47.41\% & 31.33\% & 36.64\% & 20.26\% & 20.60\%\\
\hline
\multirow{2}{*}{240}& LLR & 22.25\% & 8.53\% & 2.51\% & 24.12\% & 6.91\% & 2.28\% & 96.96\% & 72.81\% & 3.20\% & 97.89\% & 94.70\% & 2.51\%\\
\cline{2-14}
&AGR & 94.61\% & 73.73\% & 21.92\% & 96.72\% & 91.47\% & 16.67\% & 97.66\% & 86.41\% & 18.72\% & 98.13\% & 94.93\% & 15.53\%\\
\hline
\end{tabular}
\end{table*}

\begin{table*}
\def\arraystretch{1.3}
\centering
\caption{Average values of non-zero LLR/AGR over test networks.} \label{table:stat2}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
& &\multicolumn{3}{c|}{UC + Tree}&\multicolumn{3}{c|}{UC + Mesh} & \multicolumn{3}{c|}{AGC + Tree} & \multicolumn{3}{c|}{AGC + Mesh}\\
\hline
Network & $\alpha$ & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 & 0.5 & 1 & 1.5 \\
\hline
\multirow{2}{*}{118}& LLR & 1.58\% & 2.34\% & 1.05\% & 2.25\% & 2.65\% & 1.29\% & 17.69\% & 4.22\% & 3.28\% & 18.80\% & 4.64\% & 3.82\%\\
\cline{2-14}
&AGR& 10.37\% & 12.15\% & 15.68\% & 17.68\% & 15.20\% & 18.06\% & 14.56\% & 15.15\% & 16.54\% & 20.52\% & 15.38\% & 17.59\%\\
\hline
\multirow{2}{*}{179}& LLR & 1.59\% & 1.67\% & 1.71\% & 1.56\% & 1.67\% & 1.71\% & 3.33\% & 3.12\% & 2.43\% & 5.41\% & 3.16\% & 2.36\%\\
\cline{2-14}
&AGR & 26.52\% & 26.80\% & 36.71\% & 41.45\% & 42.35\% & 46.39\% & 58.30\% & 62.07\% & 38.79\% & 73.96\% & 75.15\% & 38.67\%\\
\hline
\multirow{2}{*}{200}& LLR  & 2.84\% & 2.07\% & 1.31\% & 2.35\% & 1.86\% & 1.00\% & 17.20\% & 9.94\% & 1.31\% & 13.70\% & 1.86\% & 1.00\%\\
\cline{2-14}
&AGR & 29.86\% & 36.05\% & 50.61\% & 39.94\% & 35.89\% & 50.66\% & 50.42\% & 45.43\% & 50.61\% & 49.57\% & 35.89\% & 50.66\%\\
\hline
\multirow{2}{*}{240}& LLR& 0.93\% & 1.39\% & 2.09\% & 1.00\% & 1.80\% & 2.24\% & 9.36\% & 7.19\% & 2.77\% & 9.78\% & 5.53\% & 3.34\%\\
\cline{2-14}
&AGR & 24.47\% & 21.52\% & 51.93\% & 40.62\% & 45.50\% & 66.24\% & 49.49\% & 50.42\% & 51.61\% & 60.43\% & 56.17\% & 63.12\% \\
\hline
\end{tabular}
\end{table*}













% \begin{table*}[!t]
% \def\arraystretch{1.3}
% \centering
% \caption{Number of scenarios with non-zero LLR/AGR.} \label{table:stat1}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% &\multicolumn{4}{c|}{Proposed Approach}&\multicolumn{4}{c|}{AGC}\\
% \hline
%  $(\alpha,\beta)$&$(0.8, 0.8)$ & $(0.7, 0.8)$ & $(0.65, 0.8)$ &$(0.65, 0.5)$ &$(0.8, 0.8)$ & $(0.7, 0.8)$ & $(0.65, 0.8)$ &$(0.65, 0.5)$ \\
% \hline
% LLR & 97 & 101& 123& 144 & 124 & 499 &2398 & 2476\\
% \hline
% AGR & 553& 790 & 1301& 1308 &390 & 794 & 2695 & 2744\\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[!t]
% \def\arraystretch{1.3}
% \centering
% \caption{Average values of non-zero LLR/AGR.} \label{table:stat2}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% &\multicolumn{4}{c|}{Proposed Approach}&\multicolumn{4}{c|}{AGC}\\
% \hline
%  $(\alpha,\beta)$&$(0.8, 0.8)$ & $(0.7, 0.8)$ & $(0.65, 0.8)$ &$(0.65, 0.5)$ &$(0.8, 0.8)$ & $(0.7, 0.8)$ & $(0.65, 0.8)$ &$(0.65, 0.5)$ \\
%  \hline
% LLR & 1.08\% & 1.04\% & 0.87\%& 0.98\% & 2.23\% & 6.50\% & 6.44\% & 7.92\% \\
% \hline
% AGR & 31.5\% & 28.1\% & 23.1\% & 21.9\% & 45.2\% & 58.0\% &77.6\% & 70.0\% \\
% \hline
% \end{tabular}
% \end{table*}
